Cocktail Party Attack: Breaking Aggregation-Based Privacy in Federated Learning using Independent Component Analysis

Federated learning (FL) aims to perform privacy-preserving machine learning on distributed data held by multiple data owners. To this end, FL requires the data owners to perform training locally and share the gradient updates (instead of the private inputs) with the central server, which are then securely aggregated over multiple data owners. Although aggregation by itself does not provably offer privacy protection, prior work showed that it may suffice if the batch size is sufficiently large. In this paper, we propose the Cocktail Party Attack (CPA) that, contrary to prior belief, is able to recover the private inputs from gradients aggregated over a very large batch size. CPA leverages the crucial insight that aggregate gradients from a fully connected layer is a linear combination of its inputs, which leads us to frame gradient inversion as a blind source separation (BSS) problem (informally called the cocktail party problem). We adapt independent component analysis (ICA)--a classic solution to the BSS problem--to recover private inputs for fully-connected and convolutional networks, and show that CPA significantly outperforms prior gradient inversion attacks, scales to ImageNet-sized inputs, and works on large batch sizes of up to 1024.

==> 3.preliminaries.tex <==


\section{Preliminaries}
Our paper uses ICA to break aggregation-based privacy by framing gradient inversion as a BSS problem. In this section, we formalize the objective of gradient inversion attack and provide background on BSS by using the \emph{cocktail party problem} as a motivating example.
%proposes to break aggregation-based privacy in FL by framing gradient inversion as a blind source separation (BSS) problem and using independent component analysis (ICA) to leak private inputs from aggregate gradients. . 






